Transfer Learning for the Efficient Detection of COVID-19 from Smartphone Audio Data

Disease detection from smartphone data represents an open research challenge in mobile health (m-health) systems. COVID-19 and its respiratory symptoms are an important case study in this area and their early detection is a potential real instrument to counteract the pandemic situation. The efficacy of this solution mainly depends on the performances of AI algorithms applied to the collected data and their possible implementation directly on the users' mobile devices. Considering these issues, and the limited amount of available data, in this paper we present the experimental evaluation of 3 different deep learning models, compared also with hand-crafted features, and of two main approaches of transfer learning in the considered scenario: both feature extraction and fine-tuning. Specifically, we considered VGGish, YAMNET, and L\textsuperscript{3}-Net (including 12 different configurations) evaluated through user-independent experiments on 4 different datasets (13,447 samples in total). Results clearly show the advantages of L\textsuperscript{3}-Net in all the experimental settings as it overcomes the other solutions by 12.3\% in terms of Precision-Recall AUC as features extractor, and by 10\% when the model is fine-tuned. Moreover, we note that to fine-tune only the fully-connected layers of the pre-trained models generally leads to worse performances, with an average drop of 6.6\% with respect to feature extraction. %highlighting the need for further investigations. Finally, we evaluate the memory footprints of the different models for their possible applications on commercial mobile devices.

==> fig_clf_memory.tex <==
\begin{figure*}[t]
    \begin{subfigure}[h]{0.245\linewidth}
        \centering
        \includegraphics[width=\linewidth]{kdd_1}
        \caption{Cambridge Task 1}
    \end{subfigure}
    \hfill
    \begin{subfigure}[h]{0.245\linewidth}
        \includegraphics[width=\linewidth]{kdd_2}
        \caption{Cambridge Task 2}
    \end{subfigure}
    \hfill
    \begin{subfigure}[h]{0.245\linewidth}
        \includegraphics[width=\linewidth]{kdd_3}
        \caption{Cambridge Task 3}
    \end{subfigure}
    \hfill
    \begin{subfigure}[h]{0.245\linewidth}
        \includegraphics[width=\linewidth]{coswara}
        \caption{COSWARA+Virufy}
    \end{subfigure}%
    \caption{Memory footprint of the considered shallow classifiers for each value of PCA coefficient in the different experiments.}
    \label{fig:memory}
\end{figure*}

==> tab_classification_results.tex <==
\begin{table*}[t]
\centering
\caption{Classification results}
\label{tab:classification_results}
\begin{tabular}{ccllclllll}
\toprule
Dataset & Task & Method & Modality & Features & Classifier & PCA & \multicolumn{3}{c}{Mean (\textpm~std)} \\
\midrule
& & & & & & &
\multicolumn{1}{c}{AUC} & \multicolumn{1}{c}{Precision} & \multicolumn{1}{c}{Recall} \\
\cmidrule(lr{0.5em}){8-10}
\multirow{9}{*}{Cambridge} & \multirow{3}{*}{1} &
baseline & Cough + Breath & F2 & LR & .95 & .80 (.07) & .72 (.06)  & \textbf{.69 (.11)} \\
& & our (same) & Cough + Breath  & F2 & LR & .95 & .76 (.092) & .69 (.095) & .68 (.158) \\
& & our (best) & Cough + Breath & F2 & SVM & .70 & .80 (.068) & \textbf{.77 (.096)} & .68 (.139) \\

\cmidrule(lr{0.5em}){2-10} & \multirow{3}{*}{2} &
baseline & Cough & F2 & SVM & .90 & .82 (.18) & .80 (.16) & \textbf{.72 (.23)} \\
& & our (same) & Cough & F2 & SVM & .90 & .69 (.227) & .74 (.187) & .61 (.276) \\
& & our (best) & Breath & F1 & LR & .80 & \textbf{.84 (.168)} & \textbf{.92 (.106)} & .60 (.237) \\

\cmidrule(lr{0.5em}){2-10} & \multirow{3}{*}{3} &
baseline & Breath & F3 & SVM & .70 & .80 (.14) & .69 (.20) & .69 (.26) \\
& & our (same) & Breath & F3 & SVM & .70 & .64 (.254) & .69 (.154) & .66 (.269) \\
& & our (best) & Breath & F1 & AB & .70 & \textbf{.88 (.066)} & \textbf{.82 (.152)} & \textbf{.79 (.192)} \\

\toprule

\multirow{2}{*}{COSWARA + Virufy} & &
baseline & & Top 4 & Ensemble CNN & - & .77 & .80 & .71 \\
& & our & & F3 & LR & .99 & \textbf{.99 (.001)} & \textbf{.99 (.006)} & \textbf{.99 (.007)} \\
\bottomrule
\end{tabular}

\end{table*}

==> tab_fe_results_cambridge_kdd.tex <==
\begin{table}[t]
\caption{Features extraction results with the Cambridge KDD dataset.}
\label{tab:fe_cambridge_kdd}
\resizebox{\textwidth}{!}{%
\begin{tabular}{l|crr|crr|crr}
\toprule
                     & \multicolumn{3}{c|}{\textbf{Cough}}                    & \multicolumn{3}{c|}{\textbf{Breath}}                   & \multicolumn{3}{c}{\textbf{Both}}            \\
\textbf{Features}    & \textbf{Clf} & \textbf{PCA} & \textbf{AUC} & \textbf{Clf} & \textbf{PCA} & \textbf{AUC} & \textbf{Clf} & \textbf{PCA} & \textbf{AUC}       \\
\toprule
HC                   & AB           & .60          & .78   & AB           & .80          & .85   & RF           & .60          & .83   \\
YAMNET               & LR           & .99          & .74   & SVM          & .99          & .78   & LR           & .95          & .73   \\
VGGish               & AB           & .99          & .89   & LR           & .65          & .85   & AB           & .95          & .86   \\
\midrule
L3 E 512 L           & LR           & .70          & .86            & LR           & .95          & .87   & RF           & .90          & .88   \\
L3 E 512 M128        & LR           & .60          & .85            & LR           & .85          & .88   & LR           & .80          & .86   \\
L3 E 512 M256        & RF           & .80          & .91   & SVM          & .85          & .88   & AB           & .99          & .89   \\
L3 E 6144 L          & RF           & .75          & .88            & RF           & .75          & .84            & SVM          & .99          & .86   \\
L3 E 6144 M128       & RF           & .70          & .77            & AB           & .85          & .83            & AB           & .90          & .81   \\
L3 E 6144 M256       & \textbf{LR}           & \textbf{.90}          & \textbf{.94}   & \textbf{LR}           & \textbf{.80}          & \textbf{.92}   & \textbf{LR}           & \textbf{.85}          & \textbf{.93}   \\
L3 M 512 L           & LR           & .70          & .82            & RF           & .80          & .89   & SVM          & .65          & .86   \\
L3 M 512 M128        & SVM          & .95          & .77            & SVM          & .60          & .81            & SVM          & .99          & .80            \\
L3 M 512 M256        & LR           & .95          & .86            & RF           & .95          & .87   & LR           & .90          & .89   \\
L3 M 6144 L          & LR           & .75          & .91   & SVM          & .85          & .89   & LR           & .70          & .88   \\
L3 M 6144 M128       & RF           & .90          & .93   & \textbf{LR}           & \textbf{.85}          & \textbf{.92}   & AB           & .95          & .91   \\
L3 M 6144 M256       & LR           & .65          & .92   & \textbf{LR}           & \textbf{.90}          & \textbf{.92}   & \textbf{LR}           & \textbf{.85}          & \textbf{.93}   \\
\bottomrule
\end{tabular}


}
\end{table}

==> tab_fe_results_cambridge_npj.tex <==
\begin{table}[t]
\caption{Features extraction results with the Cambridge npj dataset.}
\label{tab:fe_cambridge_kdd}
\resizebox{\textwidth}{!}{%
\begin{tabular}{l|crr|crr|crr}
\toprule
                     & \multicolumn{3}{c|}{\textbf{Cough}}                    & \multicolumn{3}{c|}{\textbf{Breath}}                   & \multicolumn{3}{c}{\textbf{Both}}            \\
\textbf{Features}    & \textbf{Clf} & \textbf{PCA} & \textbf{AUC} & \textbf{Clf} & \textbf{PCA} & \textbf{AUC} & \textbf{Clf} & \textbf{PCA} & \textbf{AUC}       \\
\toprule
HC                   & SVM          & .70          & .64        & SVM          & .99          & .62   & LR           & .70          & .63   \\
YAMNET               & SVM          & .60          & .62        & SVM          & .99          & .63   & SVM          & .75          & .63   \\
VGGish               & SVM          & .70          & .62        & SVM          & .99          & .65   & SVM          & .65          & .65   \\
\midrule
L3 E 512 L           & \textbf{SVM}          & \textbf{.75}          & \textbf{.70}& SVM          & .65         & .65   & SVM          & .65          & .63   \\
L3 E 512 M128        & SVM          & .99          & .67        & LR           & .99          & .64   & \textbf{SVM}          & \textbf{.90}          & \textbf{.67}   \\
L3 E 512 M256        & LR           & .99          & .65        & \textbf{SVM}          & \textbf{.99}          & \textbf{.67}   & SVM          & .90          & .65   \\
L3 E 6144 L          & LR           & .95          & .65        & SVM          & .80          & .63   & LR           & .80          & .65   \\
L3 E 6144 M128       & LR           & .95          & .65        & SVM          & .75          & .62   & SVM          & .85          & .66   \\
L3 E 6144 M256       & LR           & .95          & .66        & LR           & .85          & .64   & SVM          & .80          & .66   \\
L3 M 512 L           & SVM          & .95          & .65        & SVM          & .65          & .62   & SVM          & .90          & .64   \\
L3 M 512 M128        & LR           & .99          & .66        & LR           & .60          & .62   & SVM          & .80          & .64   \\
L3 M 512 M256        & SVM          & .65          & .66        & SVM          & .90          & .66   & SVM          & .75          & .64   \\
L3 M 6144 L          & SVM          & .90          & .65        & SVM          & .65          & .62   & LR           & .99          & .64   \\
L3 M 6144 M128       & LR           & .95          & .68        & SVM          & .85          & .66   & SVM          & .85          & .68   \\
L3 M 6144 M256       & LR           & .95          & .67        & SVM          & .90          & .63   & SVM          & .75          & .66   \\
\bottomrule
\end{tabular}


}
\end{table}

==> tab_fe_results_coswara.tex <==
\begin{table}[t]
\caption{Features extraction results with the Coswara dataset.}
\label{tab:fe_coswara}
\resizebox{\textwidth}{!}{%

\begin{tabular}{l|crr|crr|crr}
\toprule
                  & \multicolumn{3}{c|}{\textbf{Cough}}                    & \multicolumn{3}{c|}{\textbf{Breath}}                   & \multicolumn{3}{c}{\textbf{Both}}                     \\
\textbf{Features} & \textbf{Clf} & \textbf{PCA} & \textbf{AUC} & \textbf{Clf} & \textbf{PCA} & \textbf{AUC} & \textbf{Clf} & \textbf{PCA} & \textbf{AUC} \\
\toprule
HC                & AB           & .90          & .68            & AB           & .99          & .74            & SVM          & .65          & .70            \\
YAMNET            & RF           & .99          & .56            & LR           & .99          & .66            & RF           & .99          & .61            \\
VGGish            & RF           & .70          & .61            & RF           & .75          & .68            & SVM          & .65          & .63            \\
\midrule
L3 E 512 L        & \textbf{LR}           & \textbf{.70}          & \textbf{.73}   & RF           & .90          & .70            & AB           & .99          & .74            \\
L3 E 512 M128     & LR           & .99          & .71            & RF           & .75          & .70            & AB           & .95          & .73            \\
L3 E 512 M256     & SVM          & .85          & .68            & AB           & .95          & .71            & AB           & .85          & .72            \\
L3 E 6144 L       & LR           & .95          & .65            & LR           & .99          & .69            & LR           & .99          & .68            \\
L3 E 6144 M128    & LR           & .85          & .72            & \textbf{AB}           & \textbf{.99}          & \textbf{.76}   & SVM          & .75          & .73            \\
L3 E 6144 M256    & LR           & .75          & .72            & RF           & .85          & .74            & AB           & .99          & .71            \\
L3 M 512 L        & RF           & .70          & .71            & RF           & .85          & .73            & SVM          & .85          & .70            \\
L3 M 512 M128     & RF           & .80          & .69            & AB           & .99          & .74            & RF           & .70          & .72            \\
L3 M 512 M256     & LR           & .60          & .70            & RF           & .90          & .71            & AB           & .99          & .69            \\
L3 M 6144 L       & LR           & .75          & .70            & LR           & .99          & .70            & AB           & .95          & .72            \\
L3 M 6144 M128    & SVM          & .75          & .69            & LR           & .99          & .74            & AB           & .99          & .72            \\
L3 M 6144 M256    & SVM          & .99          & .69            & AB           & .90          & .72            & \textbf{RF}           & \textbf{.85}          & \textbf{.75}   \\
\bottomrule
\end{tabular}


}
\end{table}

==> tab_fe_results_coughvid.tex <==
\begin{table}[t]
\caption{Features extraction results with the Coughvid dataset.}
\label{tab:fe_coughvid}
\centering
\begin{tabular}{l|crr}
\toprule
                  & \multicolumn{3}{c}{\textbf{Cough}}                    \\
\textbf{Features} & \textbf{Clf} & \textbf{PCA} & \textbf{AUC} \\
\toprule
HC                & SVM          & .80          & .61            \\
YAMNET            & SVM          & .60          & .56            \\
VGGish            & LR           & .70          & .59            \\
\midrule
L3 E 512 L        & SVM          & .75          & .62            \\
L3 E 512 M128     & LR           & .99          & .67            \\
L3 E 512 M256     & LR           & .99          & .64            \\
L3 E 6144 L       & LR           & .99          & .65            \\
L3 E 6144 M128    & \textbf{LR}  & \textbf{.99} & \textbf{.68}   \\
L3 E 6144 M256    & LR           & .99          & .67            \\
L3 M 512 L        & RF           & .90          & .62            \\
L3 M 512 M128     & LR           & .99          & .62            \\
L3 M 512 M256     & LR           & .75          & .60            \\
L3 M 6144 L       & LR           & .99          & .67            \\
L3 M 6144 M128    & LR           & .99          & .65            \\
L3 M 6144 M256    & LR           & .99          & .64            \\
\bottomrule
\end{tabular}

\end{table}

==> tab_features.tex <==
\begin{table}
    \centering
    \caption{Hand-crafted acoustic features.}
    \label{tab:hc_features}
    \begin{tabularx}{\textwidth}{l X}
        \toprule
        \textbf{Feature}& \textbf{Description} \\
        \midrule
        Duration & total length (in seconds) of the audio sample, after removing possible starting and ending silence \\
        Onset & number of pitch onsets (i.e., ``events'') in the audio signal    \\
        Tempo & rate of beats that occur at regular intervals throughout the entire audio signal \\
        Period & the frequency with the highest amplitude among those obtained from the Fast Fourier Transform (FFT) \\
        RMS Energy & root-mean-square of the signal power (i.e., the magnitude of the short-time Fourier transform)  \\
        Spectral Centroid  & the centroid value of the frame-wise magnitude spectrogram. It can be used to identify percussive and sustained sounds \\
        Roll-off Frequency  & the frequency under which the 85\% of the total energy of the frame-wise spectrum is contained \\
        Zero-crossing rate  & the number of times the signal value crosses the zero axe, and it is computed for each frame   \\
        MFCC  & the shape of the cosine transformation of the sound logarithmic spectrum, expressed in Mel-bands \\
        $\Delta$-MFCC, $\Delta^2$-MFCC & the first and second order derivatives of MFCC along time \\
    \bottomrule
    \end{tabularx}
\end{table}
